Conic optimization with spectral functions on Euclidean Jordan algebras

Spectral functions on Euclidean Jordan algebras arise frequently in convex models. Despite the success of primal-dual conic interior point solvers, there has been little work on enabling direct support for spectral cones, i.e. proper nonsymmetric cones defined from epigraphs and perspectives of spectral functions. We propose simple logarithmically homogeneous barriers for spectral cones and we derive efficient, numerically stable procedures for evaluating barrier oracles such as inverse Hessian operators. For two useful classes of spectral cones - the root-determinant cones and the matrix monotone derivative cones - we show that the barriers are self-concordant, with nearly optimal parameters. We implement these cones and oracles in our open source solver Hypatia, and we write simple, natural formulations for four applied problems. Our computational benchmarks demonstrate that Hypatia often solves the natural formulations more efficiently than advanced solvers such as MOSEK 9 solve equivalent extended formulations written using only the cones these solvers support.

==> tables/centpoly.tex <==
\small
\sisetup{
table-text-alignment = right,
table-auto-round,
table-figures-integer = 4,
table-figures-decimal = 1,
table-format = 4.1,
add-decimal-zero = false,
add-integer-zero = false,
}
\begin{tabular}{crrcrScrScrS}
\toprule
& & & \multicolumn{3}{c}{Hypatia-NF} & \multicolumn{3}{c}{Hypatia-EF} & \multicolumn{3}{c}{MOSEK-EF} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12}
cone & $m$ & $k$ & {st} & {it} & {time} & {st} & {it} & {time} & {st} & {it} & {time} \\
\midrule
\multirow{14}{*}{NegEntropy}
& 1 & 15 & \underline{co} & 14 & 0.1 & \underline{co} & 19 & 7.5 & \underline{co} & 11 & 0.4 \\
& 1 & 25 & \underline{co} & 16 & 0.6 & \underline{co} & 29 & 200. & \underline{co} & 17 & 5.7 \\
& 1 & 50 & \underline{co} & 24 & 5.5 & rl & $\ast$ & $\ast$ & \underline{co} & 25 & 220. \\
& 1 & 75 & \underline{co} & 23 & 23. & sk & $\ast$ & $\ast$ & \underline{tl} & 23 & 1845. \\
& 1 & 100 & \underline{co} & 27 & 72. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 125 & \underline{co} & 29 & 167. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 150 & \underline{co} & 33 & 426. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 175 & \underline{co} & 32 & 826. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 200 & tl & 37 & 1807. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 4 & 2 & \underline{co} & 12 & 0.1 & \underline{co} & 14 & 4.0 & \underline{co} & 11 & 0.3 \\
& 4 & 3 & \underline{co} & 17 & 1.1 & tl & 19 & 1885. & \underline{co} & 22 & 27. \\
& 4 & 4 & \underline{co} & 23 & 15. & sk & $\ast$ & $\ast$ & \underline{co} & 28 & 1423. \\
& 4 & 5 & \underline{co} & 28 & 140. & sk & $\ast$ & $\ast$ & m & $\ast$ & $\ast$ \\
& 4 & 6 & \underline{tl} & 33 & 1830. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{14}{*}{NegEntropyConj}
& 1 & 15 & \underline{co} & 19 & 0.2 & \underline{co} & 44 & 16. & \underline{co} & 27 & 1.1 \\
& 1 & 25 & \underline{co} & 22 & 0.8 & \underline{co} & 53 & 376. & \underline{co} & 25 & 8.9 \\
& 1 & 50 & \underline{co} & 27 & 6.3 & rl & $\ast$ & $\ast$ & \underline{co} & 34 & 316. \\
& 1 & 75 & \underline{co} & 28 & 28. & sk & $\ast$ & $\ast$ & tl & 20 & 1822. \\
& 1 & 100 & \underline{co} & 32 & 84. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 125 & \underline{co} & 33 & 188. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 150 & \underline{co} & 34 & 423. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 175 & \underline{co} & 35 & 884. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 200 & \underline{co} & 36 & 1729. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 4 & 2 & \underline{co} & 17 & 0.1 & \underline{co} & 24 & 6.6 & \underline{co} & 14 & 0.4 \\
& 4 & 3 & \underline{co} & 24 & 1.5 & tl & 18 & 1844. & \underline{co} & 22 & 27. \\
& 4 & 4 & \underline{co} & 31 & 20. & sk & $\ast$ & $\ast$ & \underline{co} & 31 & 1477. \\
& 4 & 5 & \underline{co} & 38 & 190. & sk & $\ast$ & $\ast$ & m & $\ast$ & $\ast$ \\
& 4 & 6 & tl & 34 & 1820. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{14}{*}{Power12($1.5$)}
& 1 & 15 & \underline{co} & 16 & 0.2 & \underline{er} & 34 & 14. & \underline{co} & 15 & 0.6 \\
& 1 & 25 & \underline{co} & 22 & 0.8 & \underline{er} & 41 & 291. & \underline{co} & 19 & 6.7 \\
& 1 & 50 & \underline{co} & 31 & 7.0 & rl & $\ast$ & $\ast$ & \underline{co} & 24 & 230. \\
& 1 & 75 & \underline{co} & 38 & 38. & sk & $\ast$ & $\ast$ & tl & 22 & 1834. \\
& 1 & 100 & \underline{co} & 44 & 117. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 125 & \underline{co} & 42 & 243. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 150 & \underline{co} & 50 & 649. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 175 & \underline{co} & 54 & 1400. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 200 & tl & 37 & 1822. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 4 & 2 & \underline{co} & 16 & 0.1 & \underline{sp} & 28 & 7.7 & \underline{co} & 13 & 0.4 \\
& 4 & 3 & \underline{co} & 26 & 1.7 & tl & 18 & 1818. & \underline{co} & 18 & 24. \\
& 4 & 4 & \underline{co} & 39 & 25. & sk & $\ast$ & $\ast$ & \underline{tl} & 37 & 1820. \\
& 4 & 5 & \underline{co} & 47 & 235. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 4 & 6 & tl & 33 & 1837. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{14}{*}{Power12Conj($1.5$)}
& 1 & 15 & \underline{co} & 21 & 0.2 & \underline{co} & 43 & 16. & \underline{co} & 20 & 0.8 \\
& 1 & 25 & \underline{co} & 21 & 0.7 & \underline{co} & 60 & 412. & \underline{co} & 22 & 7.7 \\
& 1 & 50 & \underline{co} & 26 & 5.9 & rl & $\ast$ & $\ast$ & \underline{co} & 27 & 254. \\
& 1 & 75 & \underline{co} & 28 & 27. & sk & $\ast$ & $\ast$ & tl & 20 & 1826. \\
& 1 & 100 & \underline{co} & 30 & 77. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 125 & \underline{co} & 32 & 178. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 150 & \underline{co} & 35 & 430. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 175 & \underline{co} & 39 & 972. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 1 & 200 & \underline{tl} & 38 & 1821. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 4 & 2 & \underline{co} & 21 & 0.1 & \underline{co} & 37 & 10. & \underline{co} & 19 & 0.6 \\
& 4 & 3 & \underline{co} & 35 & 2.1 & tl & 18 & 1828. & \underline{co} & 25 & 33. \\
& 4 & 4 & \underline{co} & 49 & 31. & sk & $\ast$ & $\ast$ & \underline{co} & 32 & 1598. \\
& 4 & 5 & \underline{co} & 58 & 286. & sk & $\ast$ & $\ast$ & m & $\ast$ & $\ast$ \\
& 4 & 6 & tl & 34 & 1829. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\bottomrule
\end{tabular}


==> tables/classquant.tex <==
\small
\sisetup{
table-text-alignment = right,
table-auto-round,
table-figures-integer = 4,
table-figures-decimal = 1,
table-format = 4.1,
add-decimal-zero = false,
add-integer-zero = false,
}
\begin{tabular}{rcrScrScrS}
\toprule
& \multicolumn{3}{c}{Hypatia-NF} & \multicolumn{3}{c}{Hypatia-EF} & \multicolumn{3}{c}{MOSEK-EF} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
$d$ & {st} & {it} & {time} & {st} & {it} & {time} & {st} & {it} & {time} \\
\midrule
10 & \underline{co} & 17 & 0.0 & \underline{co} & 22 & 2.6 & \underline{co} & 14 & 0.5 \\
20 & \underline{co} & 21 & 0.1 & \underline{co} & 44 & 688. & \underline{co} & 19 & 14. \\
30 & \underline{co} & 22 & 0.2 & tl & 8 & 1841. & \underline{co} & 30 & 179. \\
40 & \underline{co} & 24 & 0.4 & sk & $\ast$ & $\ast$ & \underline{co} & 29 & 753. \\
50 & \underline{co} & 24 & 0.6 & sk & $\ast$ & $\ast$ & tl & 20 & 1805. \\
75 & \underline{co} & 33 & 1.8 & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
100 & \underline{co} & 34 & 3.7 & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
150 & \underline{co} & 40 & 13. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
200 & \underline{co} & 43 & 30. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
250 & \underline{co} & 42 & 57. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
300 & \underline{co} & 47 & 111. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
350 & \underline{co} & 47 & 167. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
400 & \underline{co} & 49 & 280. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
450 & \underline{co} & 53 & 420. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
500 & \underline{co} & 49 & 533. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
550 & \underline{co} & 53 & 740. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
600 & \underline{co} & 58 & 1105. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
650 & \underline{co} & 58 & 1463. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
700 & \underline{co} & 59 & 1748. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
750 & tl & 49 & 1805. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\bottomrule
\end{tabular}


==> tables/expdesign.tex <==
\small
\sisetup{
table-text-alignment = right,
table-auto-round,
table-figures-integer = 4,
table-figures-decimal = 1,
table-format = 4.1,
add-decimal-zero = false,
add-integer-zero = false,
}
\begin{tabular}{crcrScrScrS}
\toprule
& & \multicolumn{3}{c}{Hypatia-NF} & \multicolumn{3}{c}{Hypatia-EF} & \multicolumn{3}{c}{MOSEK-EF} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
cone & $d$ & {st} & {it} & {time} & {st} & {it} & {time} & {st} & {it} & {time} \\
\midrule
\multirow{13}{*}{NegRtdet}
& 25 & \underline{co} & 20 & 0.0 & \underline{co} & 14 & 0.2 & \underline{co} & 18 & 0.7 \\
& 50 & \underline{co} & 24 & 0.2 & \underline{co} & 15 & 2.7 & \underline{co} & 11 & 8.9 \\
& 75 & \underline{co} & 18 & 0.3 & \underline{co} & 15 & 13. & \underline{co} & 10 & 49. \\
& 100 & \underline{co} & 20 & 0.6 & \underline{co} & 17 & 51. & \underline{co} & 10 & 190. \\
& 150 & \underline{co} & 19 & 1.6 & \underline{co} & 17 & 357. & co & 9 & 1178. \\
& 200 & sp & 9 & 2.3 & \underline{co} & 19 & 1596. & rl & $\ast$ & $\ast$ \\
& 300 & \underline{co} & 19 & 16. & rl & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 400 & \underline{co} & 19 & 37. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 500 & \underline{co} & 23 & 95. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 600 & \underline{co} & 22 & 159. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 700 & \underline{co} & 19 & 233. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 800 & \underline{co} & 20 & 417. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 900 & \underline{co} & 18 & 554. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{13}{*}{NegLog}
& 25 & \underline{co} & 23 & 0.2 & \underline{co} & 12 & 0.2 & \underline{co} & 20 & 0.7 \\
& 50 & \underline{co} & 24 & 0.5 & \underline{co} & 13 & 2.4 & \underline{co} & 11 & 9.0 \\
& 75 & \underline{co} & 23 & 1.3 & \underline{co} & 13 & 13. & \underline{co} & 11 & 54. \\
& 100 & \underline{co} & 22 & 1.7 & \underline{co} & 13 & 40. & \underline{co} & 10 & 201. \\
& 150 & \underline{co} & 25 & 5.4 & \underline{co} & 15 & 319. & \underline{co} & 10 & 1305. \\
& 200 & \underline{co} & 21 & 10. & \underline{co} & 14 & 1199. & tl & 0 & 1853. \\
& 300 & \underline{co} & 29 & 49. & rl & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 400 & \underline{co} & 31 & 120. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 500 & \underline{co} & 39 & 297. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 600 & \underline{co} & 41 & 582. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 700 & \underline{co} & 41 & 902. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 800 & \underline{co} & 44 & 1528. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 900 & tl & 35 & 1801. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{12}{*}{NegSqrtConj}
& 25 & \underline{co} & 26 & 0.2 & \underline{co} & 14 & 0.2 & sp & 14 & 0.6 \\
& 50 & \underline{co} & 28 & 0.6 & \underline{co} & 14 & 2.4 & \underline{co} & 8 & 7.8 \\
& 75 & \underline{co} & 32 & 1.7 & \underline{co} & 15 & 12. & \underline{co} & 8 & 46. \\
& 100 & \underline{co} & 36 & 3.3 & \underline{co} & 16 & 47. & \underline{co} & 7 & 162. \\
& 150 & \underline{co} & 46 & 9.0 & \underline{co} & 19 & 382. & \underline{co} & 8 & 1170. \\
& 200 & \underline{co} & 48 & 21. & \underline{co} & 19 & 1601. & rl & $\ast$ & $\ast$ \\
& 300 & \underline{co} & 57 & 89. & rl & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 400 & \underline{co} & 66 & 233. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 500 & \underline{co} & 69 & 479. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 600 & \underline{co} & 73 & 916. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 700 & \underline{co} & 75 & 1527. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 800 & tl & 59 & 1811. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{13}{*}{NegPower($1/3$)}
& 25 & \underline{co} & 19 & 0.2 & \underline{sp} & 30 & 158. & \underline{co} & 16 & 3.4 \\
& 50 & \underline{co} & 26 & 0.6 & rl & $\ast$ & $\ast$ & \underline{sp} & 42 & 225. \\
& 75 & \underline{co} & 27 & 1.5 & sk & $\ast$ & $\ast$ & tl & 41 & 1817. \\
& 100 & \underline{co} & 24 & 2.1 & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 150 & \underline{co} & 29 & 6.3 & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 200 & \underline{co} & 27 & 13. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 300 & \underline{co} & 27 & 45. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 400 & \underline{co} & 30 & 119. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 500 & \underline{co} & 27 & 212. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 600 & \underline{co} & 29 & 420. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 700 & \underline{co} & 30 & 697. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 800 & \underline{co} & 28 & 972. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 900 & \underline{co} & 30 & 1541. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\bottomrule
\end{tabular}


==> tables/nonparam.tex <==
\small
\sisetup{
table-text-alignment = right,
table-auto-round,
table-figures-integer = 4,
table-figures-decimal = 1,
table-format = 4.1,
add-decimal-zero = false,
add-integer-zero = false,
}
\begin{tabular}{crcrScrScrScrS}
\toprule
& & \multicolumn{3}{c}{Hypatia-NF} & \multicolumn{3}{c}{Hypatia-EF} & \multicolumn{3}{c}{MOSEK-EF} & \multicolumn{3}{c}{ECOS-EF} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
cone & $d$ & {st} & {it} & {time} & {st} & {it} & {time} & {st} & {it} & {time} {st} & {it} & {time} \\
\midrule
\multirow{9}{*}{NegRtdet}
& 500 & \underline{co} & 11 & 0.0 & \underline{co} & 14 & 0.3 & co & 8 & 0.2 & \underline{co} & 22 & 0.3 \\
& 1000 & \underline{co} & 11 & 0.1 & \underline{co} & 13 & 1.5 & co & 8 & 0.7 & \underline{co} & 23 & 6.4 \\
& 2500 & \underline{co} & 12 & 0.9 & \underline{co} & 15 & 13. & co & 8 & 9.0 & \underline{co} & 23 & 107. \\
& 5000 & \underline{co} & 12 & 6.5 & \underline{co} & 14 & 68. & co & 8 & 67. & \underline{co} & 24 & 895. \\
& 10000 & \underline{co} & 10 & 49. & \underline{co} & 16 & 446. & co & 8 & 496. & tl & $\ast$ & $\ast$ \\
& 15000 & \underline{co} & 14 & 172. & \underline{co} & 14 & 1216. & co & 8 & 1589. & sk & $\ast$ & $\ast$ \\
& 20000 & \underline{co} & 15 & 404. & tl & 7 & 1863. & tl & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 25000 & \underline{co} & 14 & 756. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 30000 & \underline{co} & 13 & 1252. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{9}{*}{NegLog}
& 500 & \underline{co} & 17 & 0.1 & \underline{co} & 11 & 0.3 & \underline{co} & 8 & 0.1 & \underline{co} & 18 & 0.3 \\
& 1000 & \underline{co} & 17 & 0.2 & \underline{co} & 13 & 1.5 & \underline{co} & 16 & 0.5 & \underline{co} & 17 & 11. \\
& 2500 & \underline{co} & 25 & 1.6 & \underline{co} & 12 & 11. & \underline{co} & 8 & 3.5 & \underline{co} & 18 & 88. \\
& 5000 & \underline{co} & 29 & 11. & \underline{co} & 13 & 153. & \underline{co} & 11 & 22. & \underline{co} & 18 & 324. \\
& 10000 & \underline{co} & 36 & 85. & \underline{co} & 12 & 678. & \underline{co} & 8 & 134. & tl & $\ast$ & $\ast$ \\
& 15000 & \underline{co} & 40 & 279. & tl & $\ast$ & $\ast$ & \underline{co} & 12 & 440. & sk & $\ast$ & $\ast$ \\
& 20000 & \underline{co} & 46 & 670. & sk & $\ast$ & $\ast$ & \underline{co} & 18 & 1051. & sk & $\ast$ & $\ast$ \\
& 25000 & \underline{co} & 50 & 1331. & sk & $\ast$ & $\ast$ & \underline{tl} & 10 & 1812. & sk & $\ast$ & $\ast$ \\
& 30000 & tl & 35 & 1817. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{9}{*}{NegEntropy}
& 500 & \underline{co} & 14 & 0.0 & \underline{co} & 12 & 0.3 & \underline{co} & 17 & 0.1 & \underline{co} & 19 & 0.3 \\
& 1000 & \underline{co} & 17 & 0.2 & \underline{co} & 12 & 1.7 & \underline{co} & 13 & 0.5 & \underline{co} & 18 & 15. \\
& 2500 & \underline{co} & 24 & 1.6 & \underline{co} & 13 & 27. & \underline{co} & 19 & 4.8 & \underline{co} & 18 & 44. \\
& 5000 & \underline{co} & 28 & 11. & \underline{co} & 12 & 67. & \underline{co} & 11 & 23. & \underline{co} & 19 & 361. \\
& 10000 & \underline{co} & 35 & 84. & \underline{co} & 12 & 792. & \underline{co} & 12 & 146. & tl & 7 & 2157. \\
& 15000 & \underline{co} & 43 & 293. & \underline{co} & 11 & 1053. & \underline{co} & 8 & 420. & sk & $\ast$ & $\ast$ \\
& 20000 & \underline{co} & 45 & 663. & tl & 7 & 1861. & \underline{co} & 15 & 1003. & sk & $\ast$ & $\ast$ \\
& 25000 & \underline{co} & 50 & 1332. & sk & $\ast$ & $\ast$ & \underline{co} & 8 & 1719. & sk & $\ast$ & $\ast$ \\
& 30000 & tl & 35 & 1824. & sk & $\ast$ & $\ast$ & tl & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{9}{*}{NegSqrt}
& 500 & \underline{co} & 20 & 0.1 & \underline{co} & 10 & 0.7 & \underline{co} & 6 & 0.2 & \underline{co} & 9 & 0.2 \\
& 1000 & \underline{co} & 19 & 0.2 & \underline{co} & 10 & 3.7 & \underline{co} & 7 & 0.8 & \underline{co} & 8 & 11. \\
& 2500 & \underline{co} & 20 & 1.4 & \underline{co} & 11 & 32. & \underline{co} & 8 & 14. & \underline{co} & 8 & 161. \\
& 5000 & \underline{co} & 22 & 10. & \underline{co} & 9 & 153. & \underline{co} & 5 & 54. & \underline{co} & 8 & 343. \\
& 10000 & \underline{co} & 25 & 70. & \underline{co} & 11 & 1026. & \underline{co} & 7 & 478. & \underline{tl} & 6 & 2157. \\
& 15000 & \underline{co} & 27 & 227. & rl & $\ast$ & $\ast$ & \underline{tl} & 6 & 1966. & sk & $\ast$ & $\ast$ \\
& 20000 & \underline{co} & 32 & 555. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 25000 & \underline{co} & 36 & 1111. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
& 30000 & tl & 35 & 1821. & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ & sk & $\ast$ & $\ast$ \\
\bottomrule
\end{tabular}

